Learning Weakly-Supervised Contrastive Representations

We argue that a form of the valuable information provided by the auxiliary information is its implied data clustering information. For instance, considering hashtags as auxiliary information, we can hypothesize that an Instagram image will be semantically more similar with the same hashtags. With this intuition, we present a two-stage weakly-supervised contrastive learning approach. The first stage is to cluster data according to its auxiliary information. The second stage is to learn similar representations within the same cluster and dissimilar representations for data from different clusters. Our empirical experiments suggest the following three contributions. First, compared to conventional self-supervised representations, the auxiliary-information-infused representations bring the performance closer to the supervised representations, which use direct downstream labels as supervision signals. Second, our approach performs the best in most cases, when comparing our approach with other baseline representation learning methods that also leverage auxiliary data information. Third, we show that our approach also works well with unsupervised constructed clusters (e.g., no auxiliary information), resulting in a strong unsupervised representation learning approach.

==> fig/imagenet100.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|}
\hline
Supervision Level &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Cl-InfoNCE \\ Top-1 Accuracy (%)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Cross-Entropy\\ Top-1 Accuracy (%)\end{tabular}} &
  \multicolumn{1}{l|}{Mutual Information} &
  \multicolumn{1}{l|}{Conditional Entropy} \\ \hline
Ground Truth Supervised & 88.00         & 87.06      & 6.642 & 0       \\ \hline
Level 13                & R             & R          & 6.594 & 0       \\ \hline
Level 12                & 87.46         & eta 5 hrs  & 6.501 & 0       \\ \hline
Level 11                & 86.80         & 85.21      & 6.232 & 0       \\ \hline
Level 10                & 85.64         & 83.91      & 5.854 & 0       \\ \hline
Level 9                 & 84.90         & 82.94      & 5.603 & 0       \\ \hline
Level 8                 & 83.00         & eta 10 hrs & 4.825 & 0       \\ \hline
Level 7                 & 83.90         & eval       & 4.588 & 0       \\ \hline
Level 6                 & 80.22         & eta 3 hrs  & 3.362 & 0       \\ \hline
Level 5                 & 71.03         & 61.03      & 2.011 & 0       \\ \hline
Unsupervised InfoNCE    & with moco TBR & TBR        & 6.642 & 10.3317 \\ \hline
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}

==> fig_tex/synthetic.tex <==
\begin{figure}[t!] 
\centering
\begin{subfigure}[b]{.45\textwidth}
    \includegraphics[width=\textwidth,height=5cm]{fig/synthetic.pdf}
\end{subfigure}\quad
\begin{subfigure}[b]{.45\textwidth}
    \includegraphics[height=4.5cm, width=0.9\textwidth]{fig/synthetic_controlHorI.pdf}
    \vspace{1ex}
\end{subfigure}
\vspace{-2mm}
\caption{\small Downstream Performance versus Information Plane using Synthetic Clusters + Cl-InfoNCE on UT-Zappos50K dataset. {\bf Right:} We construct data clusters $Z$ for various information-theoretic quantities with downstream labels $T$. $I(Z;T)$ represents the mutual information and $H(Z|T)$ represents the conditional entropy. {\em SupCon} represents Supervised Contrastive Learning~\citep{khosla2020supervised} and {\em SimCLR} represents Self-supervised Contrastive Learning~\citep{chen2020simple}. {\bf Left:} We provide the plot by altering $I(Z;T)$ while having $H(Z|T)$ fixed and vice versa.}
\vspace{-4mm}
\label{fig:synthetic}
\end{figure}

==> sec/unused.tex <==



{\color{blue} four clustering approaches: 

1. clustering from attributes
attributes all are discrete. if it is a discrete variable more than 2 cardinality, we will binarize it.  

rank each attributes by entropy, and then select the top-k heighest entropy


attributes are all discrete. we first a select a number of attributes, then we construct the clusters such that the data within each have the same set of attributes (from the selected ones). changing granuality -> we increase the selected attributes, so the clusters will be more fine-grained. we will first rank each attributes by their entropy. 

2. clustering from hierarchy
original wordnet have multiple paths between parents to children. imagenet-100: choose parents only have one path. 

choosing from multiple parents to only a single parent, ensuring that there's no connected components (be care of the wordings). from the leaf node and pick the longest path.

common ancestor will be the common parents. determine the level of the common ancestor by top down.

from top to down. we will define level, our construction will ensure each level has the same hight. 


3. unsupervised k-means

iterative k-means, each epoch will update the k-means clusters

k = 25000, 50000, 100000

4. hybrid: unsupervised k-means + hierarchy

step 1: k-means determines the cluster assignments. 
step 2: identify the cluster assignments, and if the cosine similarity score's absolute value is less than 0.1, then check the cluster assignment from the hierarchy (same processing as before). 
}

%In this section we shall first discuss the technical background of the contrastive learning in unsupervised representation learning and its most representative objective - InfoNCE~\citep{oord2018representation}. Then, we will present clustering-based InfoNCE (Cl-InfoNCE), which re-formulates InfoNCE to generalize from unsupervised to weakly-supervised and supervised representation learning. Last, we will analyze the asymptotic form of Cl-InfoNCE as well as the property of the learned contrastive representations.



\subsection{Technical Background}
Contrastive learning~\citep{bachman2019learning,chen2020simple,he2020momentum} has shown its effectiveness in unsupervised representation learning, where its goal is to learn similar representations for the positively-paired (correlated) instances and dissimilar representations for the negatively-paired (uncorrelated) instances. For example, \citet{bachman2019learning,chen2020simple,he2020momentum} treat the positively-paired instances as distorted variations of the same image (e.g., the same image with different augmentations) and the negatively-paired instances as two distinct images. For another example, \citet{radford2021learning,tsai2021multiview} treat the positively-paired instances as the cross-modality pair of an instance (e.g., image and its captions) and the negatively-paired instances as pairs consisting of a random image paired with the captions of another random image. Probabilistically, we refer the positively-paired representations from the data as the representations sampled from their joint distributions (i.e., $(x,y)\sim P_{X,Y}$) and the negatively-paired representations as the representations sampled from the product of marginal distributions (i.e., $(x,y)\sim P_{X}P_{Y}$). Hence, the contrastive learning can also be interpreted as maximizing the distribution divergence between $P_{X,Y}$ and $P_{X}P_{Y}$~\citep{oord2018representation,chen2020simple,bachman2019learning,ozair2019wasserstein,tsai2021self}, and among different objectives the most popular one is maximizing the following InfoNCE objective~\citep{oord2018representation}: 
\begin{proposition}[InfoNCE~\citep{oord2018representation}]
\begin{equation}
{\rm InfoNCE}:=\underset{f}{\rm sup}\,\,\mathbb{E}_{(x_i, y_i)\sim {P_{X,Y}}^{\otimes n}}\Big[ {\rm log}\,\frac{e^{f(x_i, y_i)}}{\frac{1}{n}\sum_{j=1}^n e^{f(x_i, y_j)}}\Big]\leq D_{\rm KL}\,\big(P_{X,Y} \,\|\,P_{X}P_Y \big) = {\rm MI}\,(X,Y),
\label{eq:infonce}
\end{equation}
\end{proposition}
where $\{(x_i, y_i)\}_{i=1}^n$ are $n$ independent copies of $(x,y)\sim P_{X,Y}$, $f(x,y)$ is any function that returns a scalar from the input $(x,y)$, and ${\rm MI}\,(X,Y)$ is the mutual information (MI) between $X$ and $Y$. Practically, prior work~\citep{chen2020simple,he2020momentum} suggest $f(x,y) = {\rm cosine}(x,y) / \tau$, where ${\rm cosine}(x,y)$ is the cosine similarity and $\tau$ is the temperature hyper-parameter. Equation~\eqref{eq:infonce} suggests InfoNCE is a lower bound of ${\rm MI}\,(X,Y)$ and theoretical work~\citep{arora2019theoretical,tsai2021multiview,tosh2021contrastive} show that ${\rm MI}\,(X,Y)$ maximization could lead to representations that perform well on downstream tasks. To conclude, as the most popular contrastive approach, InfoNCE can learn good representations without the need to access the downstream supervision.

\subsection{Clustering-based Contrastive Learning}

In addition to learning without access to the downstream supervision, the contrastive learning also manifests it effectiveness under the supervised fashion~\citep{khosla2020supervised}. In particular, \citet{khosla2020supervised} present {\em Supervised Contrastive Learning} that re-defines the positively-paired samples as the samples from the same category and the negatively-paired samples as the samples belonging to different categories. Observing the fact that the contrastive learning work for both unsupervised and supervised setting, a research question pops out naturally: 

\begin{center}
{\em Can we design a unified contrastive learning objective that generalizes its applications from unsupervised to weakly-supervised and supervised representation learning?}
\end{center}

Our paper aims to answer this question by presenting clustering-based InfoNCE (Cl-InfoNCE), which 1) first constructs the clusters under either unsupervised, weakly-supervised or supervised setup and 2) then defines the positively-paired samples as the samples from the same cluster and the negatively-paired samples as the samples from different clusters. At a colloquial level, Cl-InfoNCE pulls towards the representations of the data within the same (unsupervised, weakly-supervised, or supervised-formed) cluster and push away the representations of the data from different clusters. With $Z/z$ being the constructed clusters, the proposed Cl-InfoNCE is formulated as:
\begin{proposition}[Clustering-based InfoNCE (Cl-InfoNCE)]
\begin{equation}
{\rm Cl-InfoNCE}:=\underset{f}{\rm sup}\,\,\mathbb{E}_{(x_i, y_i)\sim {\color{blue} \mathbb{E}_{z\sim P_Z}\big[P_{X|z}P_{Y|z}\big]}^{\otimes n}}\Big[ {\rm log}\,\frac{e^{f(x_i, y_i)}}{\frac{1}{n}\sum_{j=1}^n e^{f(x_i, y_j)}}\Big],
\label{eq:cl_infonce}
\end{equation}
\end{proposition}
where the positively-paired representations $(x_i, y_i)$ are sampled from ${\color{blue} \mathbb{E}_{z\sim P_Z}\big[P_{X|z}P_{Y|z}\big]}$\footnote{$(x, y) \sim \mathbb{E}_{z\sim P_Z}\big[P_{X|z}P_{Y|z}\big]$ includes two steps: first, $z \sim P_Z$; then, $x \sim P_{X|z}$ and $y \sim P_{Y|z}$.} and the negatively-paired representations $(x_i, y_j)$ are sampled from $P_XP_Y$ ($i\neq j$)\footnote{$\int_X \mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big] dx = P_Y$ and $\int_Y \mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big] dy = P_X$.}. We note that equation~\eqref{eq:cl_infonce} generalizes to different levels of supervision: 1) when $Z=$ instance id (i.e., each cluster only contains an instance), $\mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big]$ specializes to $P_{XY}$ and Cl-InfoNCE specializes to InfoNCE for unsupervised representation learning; 2) when $Z=$ downstream labels, Cl-InfoNCE specializes to the objective described in {\em Supervised Contrastive Learning}~\citep{khosla2020supervised} for supervised representation learning; and 3) when $Z$ is constructed from the weak supervision signals, such as data's attributes or the hierarchical information of data, Cl-InfoNCE can be used for weakly-supervised representation learning. Now, we provide the following theoretical statements to better understand Cl-InfoNCE:
\begin{theorem}[Asymptotic analysis of Cl-InfoNCE]
\begin{equation}
{\rm Cl-InfoNCE} \leq {\rm Cl-InfoNCE}_{\,n \rightarrow \infty} = D_{\rm KL}\,\Big( \mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big] \,\|\, P_{X}P_{Y} \Big) \leq H(Z),
\label{eq:asymp_cl_infonce}
\end{equation}
\label{theo:asymp_cl_infonce}
\end{theorem}
\begin{theorem}[Cl-InfoNCE maximization learns to include the clusering information]
\begin{equation}
{\rm Cl-InfoNCE}_{\,n \rightarrow \infty} {\rm \,\,maximizes\,\,at\,\,} H(Z) {\rm \,\,when \,\,} H(Z|X) = H(Z|Y) = 0,
\label{eq:max_resulting_repre}
\end{equation}
\label{theo:max_resulting_repre}
\end{theorem}
where $H(Z)$ is the entropy of $Z$ and $H(Z|X)$/ $H(Z|Y)$ are the conditional entropy of $Z$ given $X$/$Y$. We leave detailed derivations and proofs in Appendix. Theorem~\ref{theo:asymp_cl_infonce} suggests that Cl-InfoNCE has an upper bound $D_{\rm KL}\,\Big( \mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big] \,\|\, P_{X}P_{Y} \Big)$, which measures the distribution divergence between the product of clustering-conditional marginal distributions (i.e., $\mathbb{E}_{P_Z}\big[P_{X|Z}P_{Y|Z}\big]$) and the product of marginal distributions (i.e., $P_{X}P_{Y}$). Theorem~\ref{theo:max_resulting_repre} suggests that maximizing Cl-InfoNCE results in the representations $X$ and $Y$ including the clustering information $Z$ ($\because H(Z|X) = H(Z|Y) = 0$). This result is not surprising: since Cl-InfoNCE pulls together the representations from the data belonging to the same cluster and push away the representations from the data belonging to different clusters, the representations learned by maximizing Cl-InfoNCE should be able to distinguish among distinct clusters. 

To conclude, Cl-InfoNCE is a clustering-based contrastive learning objective. By differing its cluster construction, Cl-InfoNCE generalizes from unsupervised, weakly-supervised to supervised representation learning. In this paper, we focus on the application of Cl-InfoNCE in weakly-supervised setup, where we examine different weak supervision sources to form clusters.

==> tbl_tex/attributes-huge.tex <==

\begin{table}[t!]
\vspace{-2mm}
\centering
\scalebox{0.66}{
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{Method (Contrastive Learning$^\dagger$ / Predictive Learning$^\ddagger$)}              & \multicolumn{2}{c|}{\textbf{UT-Zappos50K}} & \multicolumn{2}{c|}{\textbf{Wider Attribute}} & \multicolumn{2}{c}{\textbf{CUB-200-2011}} \\
                                     & Top-1 Acc.              & Top-5 Acc.              & Top-1 Acc.            & Top-5 Acc.            & Top-1 Acc.               & Top-5 Acc.               \\ \midrule \midrule \multicolumn{7}{c}{\it Supervised Representation Learning} \\ \midrule \midrule
$^\ddagger$Labels + Cross-Entropy Loss                        & 89.2$\pm$0.5               & 99.6$\pm$0.4               & 44.7$\pm$1.5             & 71.2$\pm$ 0.5           & 60.5$\pm$1.2                & 81.7$\pm$0.7                \\ [1mm]
$^\dagger$(Labels + Cl-InfoNCE) SupCon~\citep{khosla2020supervised}      & 89.0$\pm$0.4                & 99.4$\pm$ 0.3              & 49.9$\pm$0.8             & 76.2$\pm$0.2             & 59.9$\pm$0.7                & 78.8$\pm$ 0.3               \\ \midrule \midrule \multicolumn{7}{c}{\it Weakly Supervised Representation Learning (Integrating Auxiliary Information into Self-supervised Representation Learning)} \\ \midrule \midrule
$^\dagger$Contrastive Multi-view Coding (CMC)~\citep{tian2020contrastive}   & 83.7$\pm$0.5                & 99.2$\pm$0.3               & 34.1$\pm$1.2          & 65.3$\pm$0.7           & 33.4$\pm$0.3                & 61.8$\pm$0.5   \\ [1mm]
$^\ddagger$Attributes-Determined Clusters + Cross-Entropy Loss   & 82.7$\pm$0.7                & 99.0$\pm$0.3               & 39.4$\pm$0.6          & 68.6$\pm$0.2           & 17.5$\pm$1.0                & 46.0$\pm$0.8   \\ [1mm]
$^\dagger$Attributes-Determined Clusters + Cl-InfoNCE (ours)      & 84.6$\pm$0.4                & 99.1$\pm$0.2               & 45.5$\pm$0.2            & 75.4$\pm$0.2             & 20.6$\pm$ 0.5               & 47.0$\pm$0.5                \\ 
%\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (clustering-based, $Z=$ unsupervised clusters)} \\ \midrule \midrule
%$^\ddagger$SwAV~\citep{caron2020unsupervised}   & xxx$\pm$xxx                & xxx$\pm$xxx               & xxx$\pm$xxx             & xxx$\pm$xxx             & xxx$\pm$xxx               & xxx$\pm$xxx   \\ [1mm]
%$^\dagger$PCL~\citep{li2020prototypical} & 82.4$\pm$0.5               & xxx$\pm$xxx               & 41.0$\pm$0.4             & xxx$\pm$xxx             & 14.4$\pm$0.5               & xxx$\pm$xxx                \\[1mm]
%$^\dagger$K-means Clusters + Cl-InfoNCE (ours)     & 84.5$\pm$0.4                & xxx$\pm$xxx               & 43.6$\pm$0.4         & xxx$\pm$xxx             & 17.6$\pm$0.2               & xxx$\pm$xxx \\
 %\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (non-clustering-based, $Z=$ instance id)} \\
  \midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning} \\
 \midrule \midrule
 $^\dagger$MoCo~\citep{he2020momentum} & 83.4$\pm$0.2                & 99.1$\pm$0.3               & 41.0$\pm$0.7             & 74.0$\pm$0.4             & 13.8$\pm$0.7               & 36.5$\pm$0.5
                \\ [1mm]
    $^\dagger$(Instance-ID + Cl-InfoNCE) SimCLR~\citep{chen2020simple} & 77.8$\pm$1.5                & 97.9$\pm$0.8               & 40.2$\pm$0.9             & 73.0$\pm$0.3             & 14.1$\pm$ 0.7               & 35.2$\pm$0.6            \\\bottomrule
\end{tabular}
}
\vspace{-1mm}
\caption{\small Experimental results under supervised (pre-training using label supervision), weakly supervised (pre-training using data attributes), and conventional self-supervised (pre-training using neither label supervision nor data attributes) setting. 
%Except for the CMC approach, each setting refers to a particular cluster construction  ($Z = $  downstream labels, attributes-determined clusters, and instance ID). 
The methods presented in this table are either contrastive or predictive learning approaches. For weakly-supervised methods that consider attributes-determined clusters, we report the best results by tuning the hyper-parameter $k$. 
}
\label{tbl:attributes-huge}
\vspace{-1mm}
\end{table}

==> tbl_tex/hierarchy.tex <==
\begin{table}[t!]
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\toprule
Supervision Level &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}\textbf{Cl-InfoNCE} \\ Top-1 Accuracy (\%)\end{tabular}} &
  \multicolumn{1}{l|}{\begin{tabular}[c]{@{}c@{}}\textbf{Cross-Entropy}\\ Top-1 Accuracy (\%)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Mutual \\ Information\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Conditional \\ Entropy\end{tabular}  \\ \midrule \midrule
Ground Truth Supervised & 88.00         & 87.06      & 6.642 & 0       \\ \hline
Level 13                & 87.80         & 86.72      & 6.594 & 0       \\ \hline
Level 12                & 87.46         & 86.83      & 6.501 & 0       \\ \hline
Level 11                & 86.80         & 85.21      & 6.232 & 0       \\ \hline
Level 10                & 85.64         & 83.91      & 5.854 & 0       \\ \hline
Level 9                 & 84.90         & 82.94      & 5.603 & 0       \\ \hline
Level 8                 & 83.00         & 79.59      & 4.825 & 0       \\ \hline
Level 7                 & 83.90         & 80.03       & 4.588 & 0       \\ \hline
Level 6                 & 80.22         & 73.86      & 3.362 & 0       \\ \hline
Level 5                 & 71.03         & 61.03      & 2.011 & 0       \\ \hline
Level 4                 & 58.21         & R      &  & 0       \\ \hline
Unsupervised InfoNCE    & 59.42 & TBR        & 6.642 & 10.3317 \\ \hline
\end{tabular}%
}
\vspace{2mm}
\caption{\small Training with Cl-InforNCE on different level of auxiliary information. {\color{red} to be deleted}} 
\label{tbl:hierarchy}
\end{table}

==> tbl_tex/unsupervised.tex <==
\begin{table}[t!]
\centering
\scalebox{0.72}{
\begin{tabular}{c|c|c|c|c}
\toprule
\multirow{2}{*}{Method}              & \multicolumn{1}{c|}{\textbf{UT-Zappos50K}} & \multicolumn{1}{c|}{\textbf{Wider Attribute}} & \multicolumn{1}{c}{\textbf{CUB-200-2011}} & \multicolumn{1}{c}{\textbf{ImageNet-100}} \\
                                     & Top-1 (Accuracy)                & Top-1 (Accuracy)             & Top-1 (Accuracy)  &   Top-1 (Accuracy)     \\ \midrule \midrule  \multicolumn{5}{c}{\it Non-clustering-based Approachs}  \\ \midrule
SimCLR~\citep{chen2020simple}       & 77.8$\pm$1.5 & 40.2$\pm$0.9       & 14.1$\pm$0.7      & 58.17$\pm$1.7  \\ [1mm]
MoCo~\citep{he2020momentum}      & 83.4$\pm$0.5               & -              & 13.84$\pm$0.5       & 59.42$\pm$1.6     \\ \midrule \multicolumn{5}{c}{\it Clustering-based Approaches} \\ \midrule
SwAV~\citep{caron2020unsupervised}   &-              & -          & -           & 69.01$\pm$2.3           \\ [1mm]
PCL~\citep{li2020prototypical}      & 82.4$\pm$0.5                & 41.0$\pm$0.4               & 14.4$\pm$0.5            & 75.92$\pm$1.3         \\ [1mm]
K-means + Cl-InfoNCE (ours)      & \textbf{84.5$\pm$0.4}               & \textbf{43.6$\pm$0.4}               & \textbf{17.6$\pm$0.2}            & \textbf{77.96$\pm$0.7}             \\ \bottomrule
\end{tabular}
}
\vspace{2mm}
\caption{\small (Comparing to unsupervised contrastive learning methods)}
\label{tbl:attributes}
\end{table}

